Towards Adaptive Mechanism Activation in Language Agent

Language Agent could be endowed with different mechanisms for autonomous task accomplishment. Current agents typically rely on fixed mechanisms or a set of mechanisms activated in a predefined order, limiting their adaptation to varied potential task solution structures. To this end, this paper proposes \textbf{A}daptive \textbf{L}anguage \textbf{A}gent \textbf{M}echanism \textbf{A}ctivation Learning with Self-Exploration (\textbf{ALAMA}), which focuses on optimizing mechanism activation adaptability without reliance on expert models. Initially, it builds a harmonized agent framework (\textbf{UniAct}) to \textbf{Uni}fy different mechanisms via \textbf{Act}ions. Then it leverages a training-efficient optimization method based on self-exploration to enable the UniAct to adaptively activate the appropriate mechanisms according to the potential characteristics of the task. Experimental results demonstrate significant improvements in downstream agent tasks, affirming the effectiveness of our approach in facilitating more dynamic and context-sensitive mechanism activation.

==> contents/introduction_0.tex <==
\section{Introduction}
Language Agent (LA) \cite{sumers2024cognitive, yao2023react, xi2023rise, gao2023large} has garnered considerable attention recently due to the rapid advancements in Large Language Models (LLMs) \cite{gpt4o, llama3modelcard, yang2023baichuan, chowdhery2022palm, radford2018improving}. Through labor-intensive strategic prompt design and in-context demonstration selection \cite{zhou2024selfdiscover, dong2023survey, liu2021pretrain},  LLMs can be endowed with different mechanisms to interact with the environment for task solving, effectively transforming them into LAs. Moreover, these LAs could benefit from distinct mechanisms for various tasks with unique solution structures \cite{zhou2024selfdiscover}. 
We define each \textbf{Mechanism} as a specific inherent ability of the Language Agent manifested as a special workflow externally and activated by the corresponding prompting.
For instance, Reflexion \cite{shinn2023reflexion} agent is equipped with \texttt{Reflection} mechanism to gain insightful refinement suggestions, ReAct \cite{yao2023react} is be equipped with \texttt{External-Augmentation} mechanism to ground the solution trajectory with additional evidence. 


% For instance, an LA might activate \texttt{Reason} \cite{wei2022chain} to arrive at the final answer step-by-step, \texttt{Plan} \cite{zhou2023leasttomost, wang-etal-2023-plan} to decompose the complex task, \texttt{Memory} \cite{sun2023expnote, gao2024retrievalaugmented} to avoid common errors, \texttt{Reflection} \cite{shinn2023reflexion, madaan2023selfrefine} to gain insightful refinement suggestions, \texttt{External Augmentation} \cite{yao2023react, schick2023toolformer} to ground the solution trajectory with additional evidence. 
%, or fine-tuning on well-curated trajectories \cite{chen2023fireact, yin2024lumos, kim2024husky},


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/main.pdf}
    \caption{Illustration of Language Agent with different mechanisms. (a). Endow vanilla agent with fixed mechanism by In-Context learning. (b) UniAct could automatically activate different mechanisms.}
    \label{fig:main}
\end{figure}

Despite the success of prompt-based LAs using \textit{manual mechanism activation} (e.g., Prompt Engineering and In-Context Learning), significant challenges persist, particularly regarding the limited accessibility of model weights for research into agent ability acquisition \cite{yao2023react, shinn2023reflexion}. As a result, the development of open-source agents has become an urgent priority. However, most fine-tuned LAs still rely on fixed mechanisms or a predefined sequence of mechanisms \cite{liu-etal-2023-plan, chen2023fireact, song2024trial}, as illustrated in Figure \ref{fig:main} (a). This rigidity hampers their adaptability to task-specific solution structures in open-world scenarios. Moreover, there is compelling evidence that \textit{oracle mechanism activation}, where the most appropriate mechanism is activated for each task, can improve performance by over 15\% compared to fixed mechanism baselines (as shown in Section \ref{sec:4.1}). We refer to this as \textbf{O}racle \textbf{L}anguage \textbf{A}gent \textbf{M}echanism \textbf{A}ctivation (\textbf{OLAMA}). This strong performance highlights the significant potential of \textit{automatic mechanism activation}, where mechanisms are adaptively activated based on task characteristics, as shown in Figure \ref{fig:main} (b). We view this as a critical meta-ability for LAs, with its enhancement offering the potential for better generalization in unseen tasks.


Each mechanism operates with its own distinct workflow. To integrate these mechanisms into a unified agent framework, this paper introduces \textbf{Uni}fy Agent Mechanisms by \textbf{Act}ions (\textbf{UniAct}). This approach defines the workflows of various mechanisms as specific actions, integrating them into a shared action space. When the agent triggers a particular action, the corresponding mechanism is activated. Unfortunately, under the zero-shot setting without fine-tuning, the current agent struggles to automatically activate the appropriate mechanisms based on task features. Intuitively, when humans encounter unfamiliar tasks, they tend to explore different strategies. When faced with similar tasks later, they select and apply the most effective methods from previous experiences. Drawing inspiration from this, the paper proposes \textbf{A}utomatic \textbf{L}anguage \textbf{A}gent \textbf{M}echanism \textbf{A}ctivation Learning with Self-Exploration (\textbf{ALAMA}), an optimization method for learning automatic mechanism activation across various tasks.

Despite the extensive efforts devoted to agent learning, current fine-tuning methods still exhibit significant shortcomings. \textbf{First}, it requires a substantial number of high-quality trajectories distilled from proprietary models for effective imitation, with unsuccessful ones often discarded \cite{zeng2023agenttuning, chen2023fireact}, leading to elevated training costs and a paucity of training signals. \textbf{Second}, exploration-based methods use success-failure pair data for behavior contrastive learning \cite{song2024trial, yuan2024advancing}. But it is training-inefficient to organize trajectories with different rewards into pair-wise format.


% 为了解决上面的问题，我们的ALAMA可以完全不依赖于专家模型的解决方案并且使用自我探索来得到不同机制激活的轨迹来进行学习。首先，我们手动激活不同的机制来进行多次自我探索，以得到同一任务的不同解决轨迹，并将这些所有轨迹统一到UnifiedAct框架下。接着，对于不同机制被激活时都能被解决的问题，我们采样出很少的一部分例子，并使用他们微调LA，以赋予他们基础的交互及指令遵循能力。最后，我们利用自我探索阶段得到的具有多样性的负例轨迹来进行偏好学习，使得LA可以对于不同的任务进行自适应机制激活。
To address these issues, our ALAMA approach does not rely on expert models but instead leverages self-exploration to obtain trajectories with different activated mechanisms for learning. Initially, we manually activate different mechanisms to facilitate multiple rounds of self-exploration, producing diverse solution trajectories for the same task. These trajectories are then converted into the UniAct format. We then sample a small subset of positive trajectories to fine-tune the LA, imparting fundamental interaction and instruction-following capabilities to the agent. Lastly, we utilize all trajectories with different rewards obtained during the self-exploration phase for behavior contrastive learning using the KTO algorithm \cite{ethayarajh2024kto}. KTO is a preference learning algorithm that only requires binary signals (desirable/undesirable), eliminating the need for assembling pairwise data. This enables the LA to dynamically activate specific mechanisms for different tasks.



% 为了验证我们提出的方法的有效性，我们在数学推理和知识密集型推理任务上进行了详尽的实验。可以与外部环境进行多轮交互以得到反馈的任务特性使得它们适合作为自动机制激活的benchmark。ALAMA可以在gsm8k上得到10/%的提升，在hotpotqa上得到了10%的提升，并且在领域外的数据集上也得到了提升，说明了我们所提出方法的先进性。
% The requirement for models to engage in multi-turn interactions with external environments to receive feedback makes these tasks suitable benchmarks for automatic mechanism activation.
% To validate the effectiveness of our proposed method, we conducted extensive experiments on mathematical reasoning \cite{cobbe2021training, mishra2022numglue, patel-etal-2021-nlp} and knowledge-intensive reasoning \cite{yang-etal-2018-hotpotqa, joshi-etal-2017-triviaqa, press-etal-2023-measuring} tasks. UniAct achieved a 6.28\% improvement on GSM8K and an 8.52\% improvement on HotpotQA, while also demonstrating strong performance gains on held-out datasets, underscoring the superiority of our approach.

Extensive experiments on mathematical reasoning \cite{cobbe2021training, mishra2022numglue, patel-etal-2021-nlp} and knowledge-intensive reasoning \cite{yang-etal-2018-hotpotqa, joshi-etal-2017-triviaqa, press-etal-2023-measuring} tasks show that UniAct surpass strong baseline by a large margin on both Held-in and Held-out datasets, demonstrating the strong performance and generalization of our proposed method.

% In summary, this paper introduces UniAct, a framework for unifying different agent mechanisms, and ALAMA, which contrasts various UniAct trajectories with different activated mechanisms to enable effective adaptability learning for agent mechanism activation.

% Our contributions are as follows:
% \begin{itemize}
   
%     \item We prose UniAct to integrate different agent mechanisms under one framework, i.e., \texttt{Reason}, \texttt{Plan}, \texttt{Memory}, \texttt{Reflection}, \texttt{External Augmentation} to interact with the environments for multiple turns for task solving.
%     \item We propose ALAMA to contrast diverse trajectories with different agent mechanisms being activated for each task to endow the LA with the ability of automatic mechanism activation.
%      \item We conduct 
% \end{itemize}










